Relativistic zero-knowledge protocol for NP over the internet unconditionally secure against quantum adversaries

Relativistic cryptography is a proposal for achieving unconditional security that exploits the fact that no information carrier can travel faster than the speed of light. It is based on space-time constraints but doesn't require quantum hardware. Nevertheless, it was unclear whether this proposal is realistic or not. Recently, Alikhani et al. [ABC+21] performed an implementation of a relativistic zero-knowledge for NP. Their implemented scheme shows the feasibility of relativistic cryptography but it is only secure against classical adversaries. In this work, we present a new relativistic protocol for NP which is secure against quantum adversaries and which is efficient enough so that it can be implemented on everyday laptops and internet connections. We use Stern's zero-knowledge scheme for the Syndrome Decoding problem, which was used before in post-quantum cryptography. The main technical contribution is a generalization of the consecutive measurement framework of [CL17] to prove the security of our scheme against quantum adversaries, and we perform an implementation that demonstrates the feasibility and efficiency of our proposed scheme.

==> new_macros.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{conjecture}{Conjecture}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{openprob}{Open Problem}
\newtheorem{remk}{Remark}
\newtheorem{apdxlemma}{Lemma}

\newenvironment{remark}{\begin{remk}

\begin{normalfont}}{\end{normalfont}
\end{remk}}
\newtheorem{sublemma}[theorem]{Sublemma}


%%%%%%%%%%%%%%%%%%%% proof environments

\def\FullBox{\hbox{\vrule width 8pt height 8pt depth 0pt}}

\def\qed{\ifmmode\qquad\FullBox\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\FullBox
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}


\newenvironment{proof}{\begin{trivlist} \item {\bf Proof:~~}}
  {\qed\end{trivlist}}


\newtheorem{fact}[theorem]{Fact}

\def\qedsketch{\ifmmode\Box\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil$\Box$
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\newenvironment{proofsketch}{\begin{trivlist} \item {\bf
Proof Sketch:~~}}
  {\qedsketch\end{trivlist}}

\newenvironment{proofof}[1]{\begin{trivlist} \item {\bf Proof
#1:~~}}
  {\qed\end{trivlist}}

\newenvironment{claimproof}{\begin{quotation} \noindent
{\bf Proof of claim:~~}}{\qedsketch\end{quotation}}


%%%%%%%%%%%%%%%%%%%%%%% text macros
\newcommand{\etal}{{\it et~al.\ }}
\newcommand{\ie} {{\it i.e.\ }}
\newcommand{\eg} {{\it e.g.\ }}
\newcommand{\cf}{{\it cf.\ }}

%%%%%%%%%%%%%%%%%%%%%%% general useful macros
\newcommand{\eqdef}{\mathbin{\stackrel{\rm def}{=}}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\N}{{\mathbb{N}}}
% \newcommand{\Z}{{\mathbb Z}}
\newcommand{\poly}{{\mathrm{poly}}}
\newcommand{\loglog}{{\mathop{\mathrm{loglog}}}}
\newcommand{\zo}{\{0,1\}}
\newcommand{\suchthat}{{\;\; : \;\;}}
\newcommand{\pr}[1]{\Pr\left[#1\right]}
\newcommand{\deffont}{\em}
\newcommand{\getsr}{\mathbin{\stackrel{\mbox{\tiny R}}{\gets}}}
\newcommand{\E}{\mathop{\mathbb E}\displaylimits}
\newcommand{\Var}{\mathop{\mathrm Var}\displaylimits}
\newcommand{\eps}{\varepsilon}
\newcommand{\KL}{\mathop{\mathrm {KL}}\displaylimits}
\newcommand{\Ent}{\mathrm H}
\newcommand{\KLb}{\mathop{\mathrm{KL_2}}}
\newcommand{\Supp}{\mathop{\mathrm{Supp}}\displaylimits}
\newcommand{\XOR}{\textsc{XOR}}
\newcommand{\OR}{\textsc{OR}}
\newcommand{\AND}{\textsc{AND}}
\newcommand{\wt}{\mathrm{wt}}
\newcommand{\Disj}{\mathop{\mathrm{Disj}}\displaylimits}
\newcommand{\mDisj}{\mathop{\mathrm{MutDisj}}\displaylimits}

%%%%%%%%%%%%%%%%%%% macros particular to this course
% for author notes
\ifnum\draft=1
\newcommand{\authnote}[2]{{ \bf [#1's Note: #2]}}
\else
\newcommand{\authnote}[2]{}
\fi
\newcommand{\Snote}[1]{{\authnote{Salil}{#1}}}
\newcommand{\Fnote}[1]{{\authnote{Florin}{#1}}}

\newcommand{\SZKOWFchar}{\textrm{SZK/OWF Characterization}}
\newcommand{\NISZKhOWFchar}{\textrm{NISZK$^h$/OWF Characterization}}
\newcommand{\NIZKbold}{\textbf{NIZK}}
\newcommand{\NISZKbold}{\textbf{NISZK}}
\newcommand{\ZKbold}{\textbf{ZK}}
\newcommand{\SZKbold}{\textbf{SZK}}

\def\textprob#1{\textmd{\textsc{#1}}}
\newcommand{\mathprob}[1]{\mbox{\textmd{\textsc{#1}}}}
\newcommand{\SAT}{\mathprob{SAT}}
\newcommand{\yes}{{\sc yes}}
\newcommand{\no}{{\sc no}}
\newcommand{\QuadRes}{\textprob{Quadratic Residuosity}}
\newcommand{\GraphIso}{\textprob{Graph Isomorphism}}
\newcommand{\GraphNoniso}{\textprob{Graph Nonisomorphism}}
\newcommand{\SZKOWFcond}{\textprob{SZK/OWF Condition}}
\newcommand{\NISZKhOWFcond}{\textprob{NISZK$^h$/OWF Condition}}
\newcommand{\NISZKcrsOWFcond}{\textprob{NISZK$^{crs}$/OWF Condition}}
\newcommand{\NISZKpubOWFcond}{\textprob{NISZK$^{pub}$/OWF Condition}}
\newcommand{\CIIDC}{\mathprob{CIIDC}}
\newcommand{\IID}{\mathprob{IID}}
\newcommand{\StatDiffUni}{\textprob{Statistical Difference from Uniform}}
\newcommand{\StatDiff}{\textprob{Statistical Difference}}
\newcommand{\CondEntApp}{\textprob{Conditional Entropy Approximation}}
\newcommand{\EntDiff}{\textprob{Entropy Difference}}
\newcommand{\EntApp}{\textprob{Entropy Approximation}}
\newcommand{\IndCond}{\textprob{Indistinguishability Condition}}
\newcommand{\CondPsEnt}{\textprob{Conditional Pseudoentropy Condition}}
\newcommand{\CondIIDCond}{\textprob{Computational Image Intersection Density Condition}}
\newcommand{\ImageInt}{\textprob{Image Intersection Density}}


\newcommand{\class}[1]{\mathrm{#1}}
\newcommand{\BPP}{\class{BPP}}
\newcommand{\NP}{\class{NP}}
\renewcommand{\P}{\class{P}}
\newcommand{\negl}{{\mathrm{neg}}}
\newcommand{\SZK}{\class{SZK}}
\newcommand{\CZK}{\class{ZK}}
\newcommand{\ZK}{\CZK}
\newcommand{\SZKh}{\class{SZK}^\mathrm{h}}
\newcommand{\CZKh}{\class{ZK}^\mathrm{h}}
\newcommand{\ZKh}{\CZKh}
\newcommand{\SZKpub}{\class{SZK}^\mathrm{pub}}
\newcommand{\CZKpub}{\class{ZK}^\mathrm{pub}}
\newcommand{\SZKcrs}{\class{SZK}^\mathrm{crs}}
\newcommand{\CZKcrs}{\class{ZK}^\mathrm{crs}}
\newcommand{\NISZKh}{\class{NISZK}^\mathrm{h}}
\newcommand{\NISZKcrs}{\class{NISZK}^\mathrm{crs}}
\newcommand{\NISZKpub}{\class{NISZK}^\mathrm{pub}}
\newcommand{\NISZK}{\class{NISZK}}
\newcommand{\NICZKh}{\class{NIZK}^\mathrm{h}}
\newcommand{\NICZKcrs}{\class{NIZK}^\mathrm{crs}}
\newcommand{\NICZKpub}{\class{NIZK}^\mathrm{pub}}
\newcommand{\NICZK}{\class{NIZK}}
\newcommand{\NIZK}{\NICZK}
\newcommand{\NIZKh}{\NICZKh}
\newcommand{\NIZKpub}{\NICZKpub}
\newcommand{\NIZKcrs}{\NICZKcrs}
\newcommand{\IP}{\class{IP}}
\newcommand{\AM}{\class{AM}}
\newcommand{\PSPACE}{\class{PSPACE}}
\newcommand{\Com}{\class{Com}}
\newcommand{\view}{\class{view}}

\newcommand{\Enc}{E}
\newcommand{\Dec}{D}
\newcommand{\Gen}{G}
\newcommand{\Tag}{M}
\newcommand{\Sign}{\mathrm{Sign}}
\newcommand{\Ver}{V}
\newcommand{\Commit}{\mathrm{Com}}

\newcommand{\MsgSp}{\mathcal{P}}
\newcommand{\KeySp}{\mathcal{K}}
\newcommand{\CiphSp}{\mathcal{C}}

\newcommand{\key}{k}
\newcommand{\td}{t}

\newcommand{\DIV}{\mathrm{DIV}}
\newcommand{\EXP}{\mathrm{EXP}}
\newcommand{\MODEXP}{\mathrm{MODEXP}}
\newcommand{\GCD}{\mathrm{GCD}}


\newcommand{\Dist}{\mathcal{D}}
\newcommand{\LR}{\mathrm{LR}}
\newcommand{\Oracle}{\mathrm{Oracle}}
\newcommand{\Adv}{\mathrm{Adv}}
\newcommand{\DES}{\mathrm{DES}}
\newcommand{\AES}{\mathrm{AES}}
\newcommand{\FFam}{\mathcal{F}}
\newcommand{\HFam}{\mathcal{H}}
\newcommand{\Rand}{\mathcal{R}}
\newcommand{\Ind}{\mathcal{I}}
\newcommand{\Dom}{D}
\newcommand{\Rng}{R}
\newcommand{\DLog}{\mathrm{DLog}}
\newcommand{\QR}{\mathrm{QR}}
\newcommand{\half}{\mathrm{half}}
\newcommand{\lsb}{\mathrm{lsb}}
\newcommand{\IV}{\mathrm{IV}}
\newcommand{\Field}{\mathbb{F}}
\newcommand{\PK}{\mathit{PK}}
\newcommand{\SK}{\mathit{SK}}
\newcommand{\pk}{\mathit{pk}}
\newcommand{\sk}{\mathit{sk}}
% \newcommand{\key}{\mathsf{key}}

\newcommand{\accept}{\mathtt{accept}}
\newcommand{\reject}{\mathtt{reject}}
\newcommand{\fail}{\mathtt{fail}}
\newcommand{\MD}[1]{\mathrm{MD{#1}}}
\newcommand{\SHA}{\mbox{SHA-1}}

\newcommand{\pf}{\mathit{proof}}
\newcommand{\compind}{\mathbin{\stackrel{\rm
c}{\equiv}}}

\newcommand{\Ideal}{\mathbf{Ideal}}
\newcommand{\Real}{\mathbf{Real}}
\newcommand{\mvec}{\overline{m}}

% Added by A.Chailloux : Quantum classes and other
\newcommand{\BQP}{\class{BQP}}
\newcommand{\QSZK}{\class{QSZK}}
\newcommand{\HVQSZK}{\class{HVQSZK}}
\newcommand{\QNISZK}{\class{QNISZK}}
\newcommand{\QNIPZK}{\class{QNIPZK}}
\newcommand{\QEA}{\textsc{QEA}}
\newcommand{\QED}{\textsc{QED}}
\newcommand{\QSD}{\textsc{QSD}}
\newcommand{\QSCU}{\textsc{QSCU}}
%\newcommand{\SCU}{\textsc{SCU}}
\newcommand{\SCUq}{\textsc{SCU}^\mathrm{q}}
\newcommand{\SD}{\mathrm{\Delta}}
\newcommand{\SC}{\mathrm{\Gamma}}
\newcommand{\SDp}{\textsc{SD}} % The promise problem SD
\newcommand{\mIID}{\mathprob{IID}}
\newcommand{\ED}{\textsc{ED}}
\newcommand{\EA}{\textsc{EA}}
\newcommand{\EAbar}{\overline{\mathprob{EA}}}
\newcommand{\SCU}{\textsc{SCU}}

\newcommand{\QNISZKh}{\class{QNISZK}^\mathrm{h}}
\newcommand{\QSZKh}{\class{QSZK}^\mathrm{h}}
\newcommand{\QAZK}{\textrm{weak-}\class{QSZK}}
\newcommand{\QNISZKch}{\class{QNISZK}^\mathrm{ch}}
\newcommand{\QNISZKhNU}{\class{QNISZK}^\mathrm{mh}}
\newcommand{\NISZKsec}{\class{NISZK}^\mathrm{sec}}
\newcommand{\IIDq}{\class{IID}^\mathrm{q}}
\newcommand{\HVSZK}{\class{HVSZK}}
\newcommand{\HVSZKq}{\class{HVSZK}^\mathrm{q}}
\newcommand{\SZKq}{\class{SZK}^\mathrm{q}}
\newcommand{\QNISZKcrs}{\class{QNISZK}^\mathrm{crs}}

\newcommand{\COMMENT}[1]{}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\ketbra}[2]{|#1\rangle\langle#2|}
\newcommand{\inp}[2]{\langle{#1}|{#2}\rangle} % inproduct, < | >
\def\01{\{0,1\}}
\newcommand{\braket}[2]{\langle{#1}|{#2}\rangle} % inproduct, < | >
\def\01{\{0,1\}}
\newcommand{\prot}[1]{\langle {#1} \rangle}
\newcommand{\triple}[3]{\langle{#1}|{#2}|{#3}\rangle}

\newcommand{\zk}{Zero-Knowledge }
\newcommand{\un}{\mathcal{U}}

\newcommand{\norm}[1]{\mbox{$\parallel{#1}\parallel$}}
\newcommand{\Tr}{\mbox{\rm Tr}}

\newcommand{\maj}[2]{\mathrm{Maj_{#1}(#2)}}
\newcommand{\wdt}[1]{\widetilde{#1}}

\newcommand{\cadre}[1]
{
\begin{tabular}{|p{15.4cm}|}
\hline
#1 \\
\hline
\end{tabular}
}

%New paper

\newcommand{\spB}{\mathcal{B}}
\newcommand{\spR}{\mathcal{R}}
\newcommand{\spH}{\mathcal{H}}
\newcommand{\spa}[1]{\mathcal{#1}}

\newcommand{\spall}{\spa{P} \otimes \spa{B} \otimes \spa{V} \otimes \spa{W}}

\newcommand{\str}{tr}

\newcommand{\css}{CS-Security }
\newcommand{\sits}{{SIT-Security }}

\newcommand{\QSZKcs}{\class{QSZK}_\mathrm{cs}}

\newcommand{\enc}{\eps}

\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\I}{\mathcal{I}}

\newcommand{\Id}{\mathbb{I}}

\newcommand{\red}{\preccurlyeq}

\newcommand{\lin}[1]{\mathcal{L}(#1)}

\newcommand{\cond}{S_c}

\newcommand{\pp}{{\textbf{P1}}}
\newcommand{\qq}{{\textbf{P2}}}

\newcommand{\Abort}{{\mathrm{Abort}}}

